The APO-K2 Catalog. I. 7,673 Red Giants with Fundamental Stellar Parameters from APOGEE DR17 Spectroscopy and K2-GAP Asteroseismology

We present a catalog of fundamental stellar properties for 7,673 evolved stars, including stellar radii and masses, determined from the combination of spectroscopic observations from the Apache Point Observatory Galactic Evolution Experiment (APOGEE), part of the Sloan Digital Sky Survey IV (SDSS), and asteroseismology from K2. The resulting APO-K2 catalog provides spectroscopically derived temperatures and metallicities, asteroseismic global parameters, evolutionary states, and asteroseismically-derived masses and radii. Additionally, we include kinematic information from \textit{Gaia}. We investigate the multi-dimensional space of abundance, stellar mass, and velocity with an eye toward applications in Galactic archaeology. The APO-K2 sample has a large population of low metallicity stars ($\sim$288 at [M/H] $\leq$ $-$1), and their asteroseismic masses are larger than astrophysical estimates. We argue that this may reflect offsets in the adopted fundamental temperature scale for metal-poor stars rather than metallicity-dependent issues with interpreting asteroseismic data. We characterize the kinematic properties of the population as a function of $\alpha$-enhancement and position in the disk and identify those stars in the sample that are candidate components of the \textit{Gaia-Enceladus} merger. Importantly, we characterize the selection function for the APO-K2 sample as a function of metallicity, radius, mass, $\nu_{\mathrm{max}}$, color, and magnitude referencing Galactic simulations and target selection criteria to enable robust statistical inferences with the catalog.

==> APO-K2 Catalog_arxix_2/table_description.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
EPIC & APOGEE ID & Campaign & Gal Lat & Gal Long & Evol & $T_{\mathrm{eff}}$ & $T_{\mathrm{eff}}$ & log(g) & log(g) \\
& & & [Deg] & [Deg] & State & [K] & Error [K] & [dex] & Error [dex]  \\
\hline
\hline
211705076 & 2M08374542+1558546 & 5,16,18 & 30.556 & 209.677 & RGB & 4664 & 7.37 & 2.87 & 0.021 \\ 
212873074 & 2M13305142-0302596 & 17 & 58.359 & 321.945 & RGB & 4789 & 11.35 & 2.78 & 0.029 \\ 
204651310 & 2M16593864-2127129 & 11 & 12.794 & 0.400 & RGB & 4667 & 7.05 & 3.03 & 0.020 \\ 
212386819 & 2M13364485-1513074 & 18,16 & 46.249 & 318.838 & RC & 4761 & 8.04 & 2.47 & 0.022 \\ 
228774437 & 2M12441419-0751315 & 10 & 54.969 & 299.824 & RC & 5006 & 9.48 & 2.85 & 0.021 \\ 
212349887 & 2M13394793-1608035 & 1 & 45.174 & 319.515 & RC & 4828 & 8.84 & 2.46 & 0.024 \\ 
204970434 & 2M16494197-2001358 & 12 & 15.510 & 0.145 & RGB & 4827 & 13.78 & 2.42 & 0.035 \\ 
228909546 & 2M12254205-0306337 & 3 & 59.131 & 290.334 & RC & 4725 & 7.78 & 2.38 & 0.0217 \\ 
...&...&...&...&...&...&...&...&...&... \\
\hline
\end{tabular}

\vspace{0.5cm}

\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
[M/H] & [Fe/H] & $[\alpha/M]$ & $\alpha$ flags & $V_{\mathrm{mag}}$ & J-K & $\nu_{max}$ & $\Delta\nu$ & $f\Delta\nu$ & $\kappa_{M}$ \\
& & & & & & $\mu$Hz & $\mu$Hz & & [$M_{\odot}$] \\
\hline
\hline
0.00 & -0.01 & 0.07 & 1 & 9.25 & 0.64 & 98.0 & 9.27 & 1.024 & 1.463 \\ 
-0.27 & -0.28 & 0.06 & 1 & 6.87 & 0.66 & 49.9 & 5.20 & 1.026 & 1.955 \\ 
0.19 & 0.17 & 0.03 & 1 & 9.60 & 0.734 & 148.6 & 12.95 & 1.016 & 1.338 \\ 
-0.05 & -0.06 & 0.01 & 1 & 9.34 & 0.64 & 33.0 & 3.95 & 0.998 & 1.686 \\ 
0.04 & 0.03 & -0.02 & 1 & 9.05 & 0.57 & 89.2 & 7.56 & 0.993 & 2.495 \\ 
-0.24 & -0.25 & 0.05 & 1 & 9.59 & 0.69 & 31.6 & 3.97 & 0.998 & 1.457 \\ 
-0.45 & -0.46 & 0.27 & 2 & 13.19 & 0.70 & 26.0 & 2.98 & 1.021 & 2.554 \\ 
-0.03 & -0.03 & -0.00 & 1 & 9.35 & 0.68 & 31.1 & 3.69 & 0.997 & 1.857 \\ 
...&...&...&...&...&...&...&...&...&... \\
\hline
\end{tabular}

\vspace{0.5cm}

\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
Mass & Mass & $\kappa_R$ & Radius & Radius & Galactic & Angular Momentum & Total Energy & $f\Delta\nu$ Flag \\
M$_{\odot}$ & Error [$M_{\odot}$] & [$R_{\odot}$] & [$R_{\odot}$] & Error [$R_{\odot}$] & Eccentricity & [kpc km s$^{-1}$] & [km$^{2}$ s$^{-2}$] & \\
\hline 
\hline 
1.06 & 0.069 & 6.776 & 6.09 & 0.125 & 0.84 & -6.5 & -2711.8 & 0 \\ 
1.48 & 0.050 & 10.974 & 9.99 & 0.111 & 0.90 & -58.3 & -2890.9 & 0 \\ 
0.97 & 0.033 & 5.262 & 4.73 & 0.053 & 0.99 & -346.9 & -2783.3 & 0 \\ 
1.26 & 0.196 & 12.540 & 11.38 & 0.575 & 0.97 & 253.4 & -2594.4 & 0 \\ 
2.01 & 0.189 & 9.273 & 8.63 & 0.261 & 0.95 & -1662.3 & -2632.9 & 0 \\ 
1.11 & 0.097 & 11.908 & 10.89 & 0.309 & 0.60 & -3263.7 & -2551.1 & 0 \\ 
1.95 & 0.217 & 17.386 & 15.89 & 0.576 & 0.85 & -2641.1 & -1960.7 & 0 \\ 
1.37 & 0.370 & 13.557 & 12.26 & 1.048 & 0.79 & -1210.8 & -2580.7 & 0 \\ 
...&...&...&...&...&...&...&...&... \\
\hline
\end{tabular}

%\begin{multicolumn}{1}
\caption{\label{tab:table_description}APO-K2 catalog. EPIC column gives the EPIC ID number for the star, and corresponds to the same row in each of the smaller tables. All observed campaigns are listed in the second column, followed by the Galactic Latitude and Longitude [degrees]. Next, we show the evolutionary state, as defined in the text as either red clump (RC) or red giant branch (RGB). The remaining columns in the top section of the table represent T$_{\mathrm{eff}}$ [K], and log(g) [dex] with their associated errors. The second section of the table gives spectroscopic abundance values from APOGEE: [M/H], [Fe/H], and [$\alpha$/M]. Next the alpha flag is given, with 1 corresponding to high [$\alpha$/Fe], 0 to low [$\alpha$/Fe], and -1 to the middle of the [$\alpha$/Fe] bimodality, with a 95\% confidence interval around the dividing line. Next, we provide the V-band magnitude and the j-k colors used in the selection function plots The final four columns of this section are the frequency of maximum oscillation power [$\mu Hz$] and large frequency separation [$\mu Hz$], followed by the f$\Delta\nu$ value. The final column of this section of the table shows the coefficient of mass [M$_{\odot}$]. The stars mass, with the coefficient used, and the appropriate error come first in the bottom section of the table, followed by the radius coefficient, stellar radius, and radius error (all [R$_{\odot}$]). Finally we provide the kinematic information from \texttt{Gala} with values of Galactic eccentricity, angular momentum and total energy. The final column is the f$\Delta\nu$ flag defined in the text. Full version available electronically, in one table.}
%\end{multicolumn}{1}


\end{table*}


